Right Time to Learn:Promoting Generalization via Bio-inspired Spacing Effect in Knowledge Distillation

Knowledge distillation (KD) is a powerful strategy for training deep neural networks (DNNs). Although it was originally proposed to train a more compact "student" model from a large "teacher" model, many recent efforts have focused on adapting it to promote generalization of the model itself, such as online KD and self KD. Here, we propose an accessible and compatible strategy named Spaced KD to improve the effectiveness of both online KD and self KD, in which the student model distills knowledge from a teacher model trained with a space interval ahead. This strategy is inspired by a prominent theory named spacing effect in biological learning and memory, positing that appropriate intervals between learning trials can significantly enhance learning performance. With both theoretical and empirical analyses, we demonstrate that the benefits of the proposed Spaced KD stem from convergence to a flatter loss landscape during stochastic gradient descent (SGD). We perform extensive experiments to validate the effectiveness of Spaced KD in improving the learning performance of DNNs (e.g., the performance gain is up to 2.31% and 3.34% on Tiny-ImageNet over online KD and self KD, respectively). Our codes have been released on github https://github.com/SunGL001/Spaced-KD.

==> imgs/Ucurve.tex <==
\begin{figure*}
    %\vspace{-.1cm}
    \centering
    \includegraphics[width=0.8\linewidth]{SPACE/imgs/figs/fig2_Ucurve.pdf}
    \vspace{-.2cm}
    \caption{Alignment of spaced learning in BNNs and DNNs. \textbf{(a)} Computational cognitive model of spaced learning, modified from~\cite{landauer1969reinforcement}. \textbf{(b)} Overall performance of Spaced KD from different networks and benchmarks. R18: ResNet-18; R50: ResNet-50; R101: ResNet-101; C100: CIFAR-100; T200: Tiny-ImageNet. \textbf{(c)} Quadratic polynomial fitting of all performance from \textbf{(b)}. %All of them show that spaced training with appropriate interval can enhance learning performance. 
    %Depiction of the cognitive model was modified from~\cite{landauer1969reinforcement}.
    }
    \label{fig:main_result}
     \vspace{-.3cm}
\end{figure*}


% /imgs/figs/\begin{figure}[t]
%     \centering
%     \begin{subfigure}{0.245\linewidth}
%     \includegraphics[width=\linewidth]{SPACE/imgs/figs/fig1_main_result_model.png}
%     \caption{Cognitive model}
%     \end{subfigure}
%     \begin{subfigure}{0.4\linewidth}
%     \includegraphics[width=\linewidth]{SPACE/imgs/figs/fig1_main_result.png}
%     \caption{Spaced KD}
%     \end{subfigure}
% \caption{\textbf{Diagram of computational cognitive model (a) of spaced learning and increased performance (b) of spaced KD.} Both of them shows spaced training is more effective than massed training, and there may be an optimal interval. The cognitive model was modified from Landauer~\citep{landauer1969reinforcement}.
% }
% \label{fig:main_result}
% \vspace{-10pt}
% \end{figure}


==> imgs/attack.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.85\linewidth]{SPACE/imgs/figs/fig_attack.pdf}
    \caption{Image corruption operation. We choose 6 representative image corruption operations with different severity (1.0, 3.0, 5.0) and visualized images come from the CIFAR-100 test set.
    }
    \label{fig: attack}
\end{figure}

==> imgs/diagram.tex <==
\begin{figure}
    \centering
     \vspace{+.2cm}
    \includegraphics[width=0.8\linewidth]{SPACE/imgs/figs/fig1_diagram.pdf}
    \vspace{-.1cm}
    \caption{\textbf{Diagram of Spaced KD.} In online KD, the teacher and student are two individual networks. In self KD, we follow the prior work~\citep{self-kd} that distills knowledge from the deepest layer to the shallower layers of the same network. In Spaced KD, we train the teacher with a controllable space interval steps ahead and then distill its knowledge to the student network.
    %Thus, the teacher is the deepest layer of the network and the students are the shallow layers along with their corresponding classifiers.
    }
    \label{fig:diagram}
    \vspace{-.4cm}
\end{figure}

==> imgs/hyperparameter.tex <==
\begin{figure} [h]
    \centering
    \includegraphics[width=0.7\linewidth]{SPACE/imgs/figs/fig5_hyperparameter.pdf}
    \caption{Hyperparameter validation for Spaced KD. Accuracy of different learning rate \textbf{(a)} and batch size \textbf{(b)} of gradient intervals. %Spaced KD is effective across all learning rates and large batch sizes.
    }
    \label{fig:hyperparameter}
\end{figure}

==> imgs/imagenet.tex <==
\begin{figure} [h]
    \centering
    \includegraphics[width=0.65\linewidth]{SPACE/imgs/figs/fig6_ImageNet.pdf}
    \caption{Training curve of ResNet-18 and ImageNet-1k (space interval 1.5 epochs).% Spaced KD remarkably improves the performance in the entire training process.
    }
    \label{fig:imagenet}
    \vspace{-.2cm}
\end{figure}

==> imgs/noise.tex <==
\begin{figure}[htb]
   % \vspace{-0.2cm}
    \centering
    \includegraphics[width=0.75\linewidth]{SPACE/imgs/figs/fig4_noise.pdf}
    \vspace{-0.01cm}
    \caption{Impact of Gaussian noise on performance. 
    % Under the same noise perturbations, the network trained with Spaced KD exhibits lower loss changes and higher accuracy.
    }
    \label{fig:noise}
    \vspace{-0.01cm}
\end{figure}
% Comparison of training accuracy and loss with increasing Gaussian noise.

==> imgs/time.tex <==
\begin{figure}[htbp!]
    \centering
    \includegraphics[width=1.0\linewidth]{SPACE/imgs/figs/fig3_time.pdf}
    % \vspace{0 pt}
    \caption{Impact of different initiating times of Spaced KD ($s=1.5$), which is introduced \textbf{(a)} for constant 10 training epochs or \textbf{(b)} till the end of training. %Spaced KD is effective at the later stage of training, rather than the early stage.
    }
    \label{fig:time}
    % \vspace{-.0cm}
\end{figure}


% Both results indicate that initiating Spaced KD in the later stages of training is more beneficial for improving the performance of the student network. This suggests that in KD learning, not only the intervals between learning sessions are important, but the timing of when learning occurs is equally crucial.

